Profiling and Modeling of Power Characteristics of Leadership-Scale HPC System Workloads

In the exascale era in which application behavior has large power & energy footprints, per-application job-level awareness of such impression is crucial in taking steps towards achieving efficiency goals beyond performance, such as energy efficiency, and sustainability. To achieve these goals, we have developed a novel low-latency job power profiling machine learning pipeline that can group job-level power profiles based on their shapes as they complete. This pipeline leverages a comprehensive feature extraction and clustering pipeline powered by a generative adversarial network (GAN) model to handle the feature-rich time series of job-level power measurements. The output is then used to train a classification model that can predict whether an incoming job power profile is similar to a known group of profiles or is completely new. With extensive evaluations, we demonstrate the effectiveness of each component in our pipeline. Also, we provide a preliminary analysis of the resulting clusters that depict the power profile landscape of the Summit supercomputer from more than 60K jobs sampled from the year 2021.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

all: sc21

.PHONY: sc21
sc21: sc21.pdf	

sc21.pdf: ./txt/*.tex ./figs/*
	pdflatex sc21.tex
	- bibtex sc21
	pdflatex sc21.tex
	- bibtex sc21
	pdflatex sc21.tex

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.fdb_latexmk \
	*.synctex.gz

clean: docclean
	$(RM) sc21.pdf
	

.PHONY: all docclean clean


==> figs/hci.tex <==
%%
%% Human Interaction with the Data
%%
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/template_single.pdf}
  \caption{\woong{Visualization}}
  %\Description{Description of the image}
  \label{figs:hci}
\end{figure}




==> tmpl/acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tmpl/acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> txt/04_05_detail_open_set.tex <==
\subsection{\ahmad{Title TBD: Open Set Detection}}
\label{subsec:details:openset}

\input{plots/example.tex}

\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}

\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}

==> txt/05_04_eval_iterative_workflow.tex <==
\subsection{Iterative Handling of Streaming Data}
\label{subsec:results:iterative_workflow}

%% TODO: Performance of the job profile database from a systems perspective Woong
%% * Evaluates ingest bandwidth, throughput and latency
%% * Evaluates inference throughput and latency

%\input{plots/example.tex}

%\woong{\loremipsum{\textbf{150-words - Evaluation 1. TBD} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

%\input{plots/example.tex}

\woong{\loremipsum{\textbf{150-words - Evaluation 2. TBD} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

==> txt/05_05_eval_applying_the_classification.tex <==
\subsection{\ahmad{Applying the Classification}}
\label{subsec:apply_classification}

%\input{tables/cluster_label_spec}
%\input{tables/label_science_domain}

We perform a cross-sectional analysis of all the jobs running on the
leadership scale HPC system to get a holistic understanding of the power consumption behavior of HPC workloads. The objective is
to find the power patterns exhibited by various jobs running on the
HPC system, and also to predict patterns of the new jobs based on the learnings from already existing jobs' characteristics. To accomplish our objective, we first generated power consumption profiles for all HPC jobs using system-level power \& temperature data and application-level job scheduler logs, as described in Table~\ref{tab:data_spec} and Table~\ref{tab:der_data_spec}. We then use the clustering methods for pattern recognition and grouping of HPC workloads' based on their power consumption behavior. 

However, we need an annotated dataset to calculate the clustering accuracy. Some techniques, such as silhouette score~\cite{rousseeuw1987silhouettes} provide metrics for cluster performance without the labeled dataset. The method measures the association between cluster cohesion and cluster separation, and its value ranges from -1 to 1. However, the silhouette score provides relative values by which we can compare various clustering methods, but it does not provide absolute metrics like cluster coherency or accuracy. Therefore, an annotated dataset is critical for reliable analysis and ensuring metrics that can assess the quality of clusters in an absolute definition. 
To address the challenge of having annotated labels, we manually labeled around $846$ power timeseries of various patterns and assigned them to different classes. We, the researchers, did the annotation independently and then compared labels assigned to these timeseries. We kept the same label for the timeseries, where we assigned the same labels unanimously. For timeseries that were assigned conflicting labels, we labeled them based on the discussion.

We randomly selected and annotated $846$ timeseries of the HPC workload. The annotation or labeling of jobs was done at four levels. Sample timeseries with classification labels are shown in Figure~\ref{figs:sample-ts}. For example, Figure~\ref{figs:sample-ts}(a) has the label FF3-2, where FF3 corresponds to the profile pattern, and 2 corresponds to a magnitude of 2000 Watts. Every alphanumeric character corresponds to a level in the assigned classification label. In Figure~\ref{figs:sample-ts}(b), the class label is FP1-2, so at level L1, the annotation is F which is similar to the label of timeseries in Figure~\ref{figs:sample-ts}(a).  At level L2, in Figure~\ref{figs:sample-ts}(b) the annotation is FP, which differs from Figure~\ref{figs:sample-ts}(a). At level L3, the class label is FP1, and at level L4, the class label is FP1-2. The first three levels (L1, L2, L3) are based on the patterns, such as rising and falling swings and slopes. Labeling of level L4 is strictly based on the magnitude of the major region in the timeseries. L1 is the high-level or more coarse-grained level, and L2, L3 \& L4 are more fine-grained levels. The hierarchical classification of the dataset has several advantages. It enables us to visualize the classification of jobs at multiple resolutions. The L1 or high-level classifies the dataset into broader patterns and captures the most salient features exhibited by the HPC jobs. As we increase the classification level from L1 to L3, the basis of difference among the timeseries becomes more nuanced, capturing more subtle patterns in the timeseries. Finally, at level L4, if the two timeseries have a similar pattern but have different magnitudes, they are grouped into different classes depending on the magnitude. For the magnitude of timeseries, we have groups of 1, 2, 3, 4, 5, 6, and 7 for magnitudes of 2500W, 2000W, 1500W, 1200W, 1000W, 800W, and 600W respectively. For example, if we look at the plots in Figure~\ref{figs:sample-ts}, some plots are more similar compared to others. If we look closely, Figure~\ref{figs:sample-ts}(a) and Figure~\ref{figs:sample-ts}(b) have similar labels and belong to group F at L1, but at L4, their groups are FF3-2 and FP1-2, respectively. Similarly, Figure~\ref{figs:sample-ts}(c) and Figure~\ref{figs:sample-ts}(d) are similar at the L1 level as both belong to the J group, but as they are not exactly similar, Figure~\ref{figs:sample-ts}(c) at L4 is assigned JJ3-2 class Figure~\ref{figs:sample-ts}(d) is assigned JJ1-2 class. 

A summary of the class description of the four-level classification is given in Table~\ref{tab:describing_cluster_labels}. We also show the distribution of 846 samples across different groups at level L1 and the number of subgroups at L3 under each L1 group.
We also show the distribution of jobs from different science domains for level L1 in Table~\ref{tab:labeling_cluster_labels}. The distribution of jobs based on the science domain helps us understand at a high-level, the dominant power profiles exhibited by different areas.

==> txt/artifact_description.tex <==

\section{Artifact Description}
\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}
%\renewcommand{\thesubsection}{\arabic{subsection}}

\subsection{Artifact Identification}
%START_LATEX
\textbf{Title}: Machine Learning Assisted Profiling of Jobs Power Consumption Timeseries for Large Scale HPC System\\
\textbf{Authors}: Ahmad Maroof Karimi, Naw Safrin Sattar, Woong Shin, Feiyi Wang \\
\textbf{Affiliation}: Oak Ridge National Laboratory\\
\\
The main contribution of the paper is the data-driven end-to-end pipeline designed and developed for processing, managing, and classification of power profiles of the system-wide workloads of a large-scale HPC system. 
Major tasks accomplished by the end-to-end workflow pipeline shown in Figure 2 of the paper are: 1) power \& energy and jobs data collection, 2) processing raw data, 3) storing the processed data in the low latency distributed database, 4) feature extraction, 5) latent feature generation 6) hierarchical classification labeling, and 7) calculating clustering and prediction quality. A brief description of the tasks is as follows:

\begin{itemize}
	\item Data Collection: We collect raw compute-node level power data and job scheduler logs; collected logs for all the workloads in the year 2021, consisting of over 1.5 million jobs (shown in Table 1 of the article).
	\item Data processing: In this stage, raw power and energy data, which is system-level data, is synced with application-level jobs logs. The processed data are listed in Table 2 in the paper.
    \item Data storage: For low latency and high availability of timeseries data, we used the Apache Druid database to store all the processed data, described in Table 2 of the paper.
	\item Features extraction: The processed data is 10 sec—interval timeseries for every job. Thus the length of the timeseries depends on the duration for which the job ran. In the feature extraction step, we extract features related to magnitude and swings/changes in the timeseries. We have summarized the list of features we extracted in Table 3 of the paper. This appendix presents the feature list with a more detailed description in Table \ref{tab:ftr_apndx_tbl}.
    \item Latent feature generation: Latent feature generation using the GAN model has several advantages in the analysis and modeling of the power profiles. We have leveraged it here to reduce the dimensionality of the feature set to enable better clustering scores.
	\item Hierarchical classification labeling: The significance of this task is to enable us to validate and assess the quality of the machine learning methods we used. Although we processed and performed clustering of about 60K jobs, we labeled 846 random samples to calculate and report the cluster quality and prediction quality in this task. As described in Section 4.4 of the paper, we did hierarchical labeling in four levels (L1, L2, L3, and L4). Hierarchical labels enabled us to look at the power patterns exhibited by jobs at multiple granularities. A summary of the classification label is shown in Table 4 of the article. Table~\ref{tab:class_level_labels} shows the number of high-level classes at L1 and subclasses at levels L2 L3, and L4. 
    \item Clustering and Prediction: We identify and classify power profiles exhibited by HPC jobs into different classes at different resolution levels. The clustering and prediction quality scores are reported in sections 5.1 and 5.2, respectively.
    \end{itemize}

While the primary artifact is essentially an end-to-end data pipeline, artifacts resulting from this work also include a framework and a set of infrastructure-level building blocks dedicated for use to support such a data pipeline.
Implemented in the forms of in-house re-usable python libraries, the framework supports data pipeline artifacts which are implemented and deployed as either containerized persistent applications or a workflow, connecting and orchestrating several infrastructure-level building blocks we have deployed for this work.  These building blocks provide the ability to efficiently utilize the necessary compute, memory, and storage while handling large volumes of data involved.  Mainly depicted in Figures 2 and 3 in Section 3, such infrastructure-level building blocks include the following:

\begin{itemize}
    \item Minio, an S3 interface-based object storage to store archived historical data or intermediate data for batch processing as well as providing backend persistence for other building blocks
    \item Apache Druid, a timeseries database to serve downstream interactive workloads via REST APIs or web applications
    \item Apache Spark-based data analytics cluster for both batch and stream data processing
    \item MLFlow, an experiment tracker and model registry for machine learning model development and maintenance
    \item Apache Airflow, a workflow orchestration engine to perform batch processing orchestration of workflows
    \item RedisAI, an inference server for GPU usage consolidation for online inference
    \item Jupyterhub, a multi-tenent jupyter notebook server provider to support the interactive needs of the authors in developing and managing the data pipelines and experiments
\end{itemize}

The artifacts of this work include a wide array of components required for high-performance data processing and data-intensive machine learning modeling tasks.  However, the system still relies on several external systems and services provided to the authors from other groups in our organization. These systems and services are not scoped as artifacts from this work. Such items are as the following:

\begin{itemize}
    \item Center-wide Kubernetes cluster which all the artifacts are deployed and operated on top of
    \item The data engineering and distribution system depicted in Figure 1 provides a unified interface to a wide array of data streams coming from heterogeneous data sources
\end{itemize}

The computational artifacts (dataset and workflow pipeline/code) have a major role in enabling us to develop a system for profiling and classifying power profiles of all workloads on the HPC machine. The results presented in the paper are the direct outcome of the workflow presented here. 

\begin{table}
    \caption{Features extracted from timeseries of power profiles of each job. The features prefixed with $1\_$ represent the features calculated for the first bin. We similarly calculate features for the other three bins, not shown here for brevity. The four bins are created by partitioning the timeseries into 4 parts across the length of the timeseries}
    \label{tab:ftr_apndx_tbl}
    \footnotesize

    \begin{tabular}{ll}
        \toprule
        Features & Description \\
        \midrule
        allocation\_id & jobs allocation id \\
        total\_mean & mean input power of full timeseries \\
        length & length of the timeseries \\
        1\_mean\_inp\_power & mean input power \\
        1\_median\_inp\_power & median input power \\
        1\_sfqp\_25\_50 & no. of up swings from 25 to 50W \\
        1\_sfqn\_25\_50 & no. of down swings from 25 to 50W \\
        1\_sfql2p\_25\_50 & no. of up swings from 25 to 50W over 2 time-period \\
        1\_sfql2n\_25\_50 & no. of down swings from 25 to 50W over 2 time-period \\
        1\_sfqp\_50\_100 & no. of up swings from 50 to 100W \\
        1\_sfqn\_50\_100 & no. of down swings from 50 to 100W \\
        1\_sfql2p\_50\_100 & no. of up swings from 50 to 100W over 2 time-period \\
        1\_sfql2n\_50\_100 & no. of down swings from 50 to 100W over 2 time-period \\
        1\_sfqp\_100\_200 & no. of up swings from 100 to 200W \\
        1\_sfqn\_100\_200 & no. of down swings from 100 to 200W \\
        1\_sfql2p\_100\_200 & no. of up swings from 100 to 200W over 2 time-period \\
        1\_sfql2n\_100\_200 & no. of down swings from 100 to 200W over 2 time-period \\
        1\_sfqp\_200\_300 & no. of up swings from 200 to 300W \\
        1\_sfqn\_200\_300 & no. of down swings from 200 to 300W \\
        1\_sfql2p\_200\_300 & no. of up swings from 200 to 300W over 2 time-period \\
        1\_sfql2n\_200\_300 & no. of down swings from 200 to 300W over 2 time-period \\
        1\_sfqp\_300\_400 & no. of up swings from 300 to 400W \\
        1\_sfqn\_300\_400 & no. of down swings from 300 to 400W \\
        1\_sfql2p\_300\_400 & no. of up swings from 300 to 400W over 2 time-period \\
        1\_sfql2n\_300\_400 & no. of down swings from 300 to 400W over 2 time-period \\
        1\_sfqp\_400\_500 & no. of up swings from 400 to 500W \\
        1\_sfqn\_400\_500 & no. of down swings from 400 to 500W \\
        1\_sfql2p\_400\_500 & no. of up swings from 400 to 500W over 2 time-period \\
        1\_sfql2n\_400\_500 & no. of down swings from 400 to 500W over 2 time-period \\
        1\_sfqp\_500\_700 & no. of up swings from 500 to 700W \\
        1\_sfqn\_500\_700 & no. of down swings from 500 to 700W \\
        1\_sfql2p\_500\_700 & no. of up swings from 500 to 700W over 2 time-period \\
        1\_sfql2n\_500\_700 & no. of down swings from 500 to 700W over 2 time-period \\
        1\_sfqp\_700\_1000 & no. of up swings from 700 to 1000W \\
        1\_sfqn\_700\_1000 & no. of down swings from 700 to 1000W \\
        1\_sfql2p\_700\_1000 & no. of up swings from 700 to 1000W over 2 time-period \\
        1\_sfql2n\_700\_1000 & no. of down swings from 700 to 1000W over 2 time-period \\
        1\_sfqp\_1000\_1500 & no. of up swings from 1000 to 1500W \\
        1\_sfqn\_1000\_1500 & no. of down swings from 1000 to 1500W \\
        1\_sfql2p\_1000\_1500 & no. of up swings from 1000 to 1500W over 2 time-period \\
        1\_sfql2n\_1000\_1500 & no. of down swings from 1000 to 1500W over 2 time-period \\
        1\_sfqp\_1500\_2000 & no. of up swings from 1500 to 2000W \\
        1\_sfqn\_1500\_2000 & no. of down swings from 1500 to 2000W \\
        1\_sfql2p\_1500\_2000 & no. of up swings from 1500 to 2000W over 2 time-period \\
        1\_sfql2n\_1500\_2000 & no. of down swings from 1500 to 2000W over 2 time-period \\
        1\_sfqp\_2000\_3000 & no. of up swings from 2000 to 3000W \\
        1\_sfqn\_2000\_3000 & no. of down swings from 2000 to 3000W \\
        1\_sfql2p\_2000\_3000 & no. of up swings from 2000 to 3000W over 2 time-period \\
        1\_sfql2n\_2000\_3000 & no. of down swings from 2000 to 3000W over 2 time-period\\
        \bottomrule

    \end{tabular}
\end{table}

\begin{table}
    \caption{The number of classes at different levels of classification. L1 is the highest level of classification, and there are 12 high-level classes.}
    \label{tab:class_level_labels}
    \footnotesize

    \begin{tabular}{cccc}
    \toprule
    L1 & L2 & L3 & L4 \\
    \midrule
    \begin{tabular}[c]{@{}l@{}}High-level\\ classification\end{tabular} & \multicolumn{3}{l}{Sub-classes} \\
    \midrule
    A & 1 & 1 & 1 \\
    B & 1 & 2 & 2 \\
    C & 1 & 2 & 3 \\
    D & 1 & 4 & 4 \\
    F & 5 & 26 & 41 \\
    G & 5 & 14 & 22 \\
    H & 2 & 8 & 12 \\
    J & 2 & 5 & 6 \\
    L & 1 & 1 & 1 \\
    M & 1 & 2 & 3 \\
    N & 1 & 3 & 3 \\
    O & 2 & 2 & 2\\
    \bottomrule
    \end{tabular}
\end{table}
%STOP_LATEX


\subsection{Reproducibility of Experiment}:
%START_LATEX
\subsubsection{Description of the Experiment Workflow}
The end-to-end pipeline shown in Figure 2 represents the major steps involved in the framework. In the data ingestion task, we have collected system-level data and job allocation logs. During the data processing stage, we developed Python based Apache Spark scripts for processing a large amount of data by leveraging Apache Spark's distributed computing techniques for efficient processing.  After data processing, we ingest the processed data into the Apache Druid timeseries database for online interactive consumption, and also into the object store in an archived form (i.e., Apache Parquet files leveraging the Snappy algorithm) for long-term batch processing.
Mainly using the archived data for efficient batch processing, we extracted features from the processed data for a system-wide cross-sectional analysis and modeling of jobs' power profiles. The summarized list of the features is shown in the paper in Table 3. A more descriptive list of features is given here in Table \ref{tab:ftr_apndx_tbl}.
The list of features extracted is fed into the GAN model shown in Figure 5 to generate latent features of size 20. The GAN model helps reduce the dimensionality of the data and simultaneously preserves the information contained in the data. The dimensionally reduced data is used for machine learning tasks such as clustering. 
Although we cluster about 60K jobs, for calculating and reporting cluster quality scores, we labeled 846 jobs. The labeling of datasets enabled us to measure the quality of different methods in absolute numbers instead of clustering metrics such as the Silhouette score. The labeling of the cluster is accomplished at 4 resolution levels. At level-1 or L1, shown in Table 5 in the paper, we classify the datasets into 12 classes. At higher resolutions, such as at levels L2, L3, and L4, the 12 main classes at L1 are further classified into many subclasses. We report the cluster homogeneity scores in section 5.1 of the paper. In another experiment, we partition the labeled dataset into two sets of 80\% and 20\% using scikit-learn stratified-kfold cross-validation method. We use the k-means to cluster on 80\% of the data. Then we use the k-means center to predict the classes or groups of 20\% of the data based on the proximity with the cluster center. We report the results of the homogeneity score on 20\% of the data in section 5.2 of the paper. 
% \begin{itemize}
%     \item Dataset
%     \begin{enumerate}
%         \item Raw Dataset
%         \item Processed Data
%         \item Extracted Features

%     \end{enumerate}
%     \item Workflow
%     \begin{enumerate}
%         \item 
%     \end{enumerate}    
% \end{itemize}


\subsubsection{Execution Time to Execute the Experiment Workflow}
\textit{Data-processing}: The execution time of the initial historical data processing is 3 minutes per day of data. This makes up about 19 hours for a year's worth of data on our Spark cluster using 128-cores and 512GB memory.
\textit{Feature extraction}: The feature extraction step takes about 1 minute per day of data or 6 hours per year.  This task was executed on the Spark environment using 42 cores and 8 GB of memory per executor.
\textit{Latent feature generation by GAN}: Each epoch takes about 40 seconds, and we run it for 1000 epochs needing about 10 hours. The GAN model was developed using Python's pytorch library. The task was executed on single a node having 8GB partition of an Nvidia A100 leveraging its multi-instance GPU feature, 16 CPU cores, and 16 GB memory.  
\textit{Evaluation}7: We filtered and randomly selected 846 jobs and labeled them by hand. Labeled data was used for evaluating clustering and prediction quality. The clustering algorithms and subsequent prediction were performed on a single-node machine in a Python environment using scikit-learn python packages. The evaluation task's overall execution time on 16 cores, 16 GB memory is about 90 seconds. 

\subsubsection{A Complete Description of the Expected Results and Evaluation}
The results generated by the workflow are much more comprehensive than what we reported in the article because of the space constraint. For clustering methods in k-means and DBSCAN, we explored a broad range of search spaces. For k-means, we ran the experiments with a value of K ranging from 60 to 120. Similarly, we ran DBSCAN with different combinations of the two parameters: 1) epsilon values and 2) minimum samples, as shown in Table~\ref{tab:dbscan_grid_search}.
To maintain the repeatability of results for k-means, we fixed the random\_state parameter of the k-means function. For DBSCAN we pass the data in the same order to maintain the deterministic property of the results. 

\begin{table}
    \caption{DBSCAN Grid Search Space}
    \label{tab:dbscan_grid_search}
    \footnotesize

    \begin{tabular}{cc}
    \toprule
    Epsilon & Minimum Samples \\
    
    
    \midrule
0.880 & 5      \\
0.880 & 10     \\
0.880 & 15     \\
0.881 & 5      \\
0.881 & 10     \\
0.881 & 15     \\
0.882 & 5      \\
0.882 & 10     \\
0.882 & 15     \\
0.883 & 5      \\
0.883 & 10     \\
0.883 & 15     \\
0.884 & 5      \\
0.884 & 10     \\
0.884 & 15     \\
0.885 & 5      \\
0.885 & 10     \\
0.885 & 15     \\
0.886 & 5      \\
0.886 & 10     \\
0.886 & 15     \\
0.887 & 5      \\
0.887 & 10     \\
0.887 & 15     \\
0.888 & 5      \\
0.888 & 10     \\
0.888 & 15     \\
0.889 & 5      \\
0.889 & 10     \\
0.889 & 15    \\
    \bottomrule
    \end{tabular}
\end{table}


The homogeneity scores of the clustering results are calculated for all values of K from 60 to 120 in the k-means cluster method, and all combinations of the parameters, shown in Table \ref{tab:dbscan_grid_search} for the DBSCAN method. The homogeneity scores are calculated for different resolution levels, i.e., L1, L2, L3, and L4 levels of power profile classification. 
For example, in section 5.1 of the paper, we report the result of k-means only for the K value, corresponding to the number of distinct labels at level-3. The number of classes at level-3 is 70 and the reason to choose the value of K. We do this because at level L4 there are over 100 classes and few datapoints in one class, contrary to that levels L1 and L2 are too coarse-grained. Thus, level L3 provides the right balance of classification based on the power profile patterns.

For prediction results, presented in section 5.2, we run the k-means clustering technique on stratified-kfold cross-validation method for different values of K. We save the homogeneity score in a matrix. Rows in a matrix correspond to class labels and columns represent the value of K. For each class/label for a value of K, we save the homogeneity score in a cell corresponding to the class label and K. 

\subsubsection{How Experiment Workflow Relate to the Results Found in the Article}
The results presented in the paper are the final outcomes of the workflow pipeline. The two main results are: 1) clustering to find the patterns exhibited by jobs running on the HPC system, and 2) prediction using the clustering methods for the jobs that have not been exposed to clustering algorithms. In the clustering approach, we apply k-means and DBSCAN. For both algorithms, the workflow is designed to run over a large search space. 
The output generated by the workflow is in the matrix. Each column of the matrix contains the labels assigned by the clustering method to the data. For k-means, the result matrix includes 60 columns and 846 rows. Each column corresponds to the value of K from 60 to 119. For DBSCAN, the output from the workflow matrix has 30 columns and 846 rows.  

The clustering results shown in the article in section 5.1 corresponds to the homogeneity score calculated on one column of the k-means matrix for which the value of $K=70$, and for the DBSCAN method, the results in the paper is from a column in the DBSCAN matrix that corresponds to parameter values $epsilon=.889$ and minimum sample per class as $mininmum\_sample=10$.
The plots in Figures 8 to 11 are the line plots of the power values and are grouped based on clustering results corresponding to column $K=70$ for the k-means matrix. For the DBSCAN matrix, the line plots are from the column corresponding to $epsilon=.889$ and $mininmum\_sample=10$.

The prediction results shown in section 5.2 is from k-means cluster after partitioning the data into 80\% for clustering and 20\% for prediction. 
The prediction output generated for different levels is stored in a matrix format. Different K values correspond to the columns and the 20\% test samples correspond to the number of rows. The value in each cell of the result matrix represents the prediction label of a sample job for a particular K value. Based on the actual number of classes in different granularity levels (L1, L2, L3, L4), we choose the K values ranging between $\pm 5$ of the actual number of classes. We calculate the homogeneity score using the real class labels and the predicted labels of all the test job samples for all K values. In Table 7 in the article, we only report the score that corresponds to the actual number of classes in levels L1, L2, L3, and L4. 

The heat-map in Figure 12 represents the class-wise homogeneity score for different values of K at four different classification levels corresponding to four heat-maps. At different classification levels, the class-wise homogeneity scores are stored in the matrix format where the number of rows is the actual classes, and the columns are different K values. These 4 output matrices are used to generate the heat-maps.

%STOP_LATEX

==> txt/backup/01_intro.tex <==
\section{Introduction}
\label{sec:intro}

As we are entering the exascale era, the power and energy footprint of modern supercomputers and the applications they run has grown to an unprecedented level.  To deal with the power and energy of exascale computing is a significant challenge in acquiring an exascale class supercomputer, and it is also challenging to sustain such a system throughout its lifetime at a reasonable operational cost.  With this large footprint, beyond meeting the performance goals, HPC sites also have to take energy, a physical metric, into account when setting efficiency goals \cite{ref:4pillar:2014}.

In attacking these goals, understanding the behavior of large scale HPC applications is a critical step since applications themselves drive the power-hungry compute components.  Algorithmic behavior at the code level, at scale, translates directly into a power envelope of a few tens of megawatts that have a profound impact on how the underlying HPC data center responds in terms of power distribution, cooling, and long-term reliability \cite{shin2021revealing}.  Being able to profile applications by systematically putting power and energy measurements into a subcluster level application context can both benefit existing supercomputer operations and enable cross-layer use cases especially leading toward energy-aware resource utilization at the system, software, and building infrastructure levels.  Again, it can help application developers prepare for the challenging future of post-exascale supercomputing where we would be limited by the limits of silicon technology \cite{dennards:1974, amd-supercomputer-gains:2023}.

\rev{
However, systematically acquiring such power profiles is a non-trivial task due to the sheer scale of the data that comes out from these large systems.  Also, per node, power measurements and job allocation information usually come from different sources, which makes it furthermore difficult to combine and process.  And even if one successfully acquires such data streams in one place, the sheer volume and velocity of these data streams make it difficult to parse and understand, which has been a hurdle to justify and implement in practice.  While making use of fine-grained power profiles per application has been researched to be beneficial during the lifetime of the supercomputer~\cite{naghshnejad2018adaptive,galleguillos2018data,wyatt2018prionn,mckenna2016machine,emeras2017evalix,sirbu2016power,matsunaga2010use,galleguillos2020accasim,klusavcek2020alea}, such profile information has been limited to a granular level, or created after the fact nearing the end of a relatively short  life span of supercomputers for long term retrospective analysis \cite{dennards:1974}.
}
 
\rev{To this end, we have built a job power profiling and clustering system that can classify the entirety of jobs executed at scale by processing streaming telemetry data.  Especially, targeted for pre-exascale and exascale supercomputers such as \hpc~\cite{summit} and \hpd~\cite{frontier}, the system operates on streams of high-resolution high-volume out-of-band power and energy measurements per component data~\cite{shin2021revealing, Thaler:2020, openbmc_event} from these systems and generates 10-second interval job and component level time series power profiles put in various levels (job, node, component), augmented by unsupervised machine learning based grouping information (clusters) based on similarities found in many features of the job-level timeseries.}

\rev{This is achieved by designing a data-driven machine learning pipeline that operates on streaming data, powered by several distributed stream processing building blocks to perform the necessary joining, indexing, and reduction of multiple data streams down to a form in which low-latency access and bulk access from downstream applications are possible.  Leveraging the indexed output, we have implemented an unsupervised machine learning-based clustering pipeline that extracts 187 features from the timeseries to train a k-means clustering-based predictor, whose purpose is to perform job classification at lower latency and higher throughput.  Due to the high-dimensional nature of the data, a generative adversarial network (GAN)~\cite{tadgan, clustergan, gan8594983} reduces its dimensionality and helps with the clustering.  With occasional offline processing \& training from long-term historical data, the predictor can perform near-real time classification of the incoming jobs considering all existing prior known jobs that have been executed before.  The indexed data and the group information are then stored and served as a common resource to power many downstream applications.
With this system, our contributions are as the following:}

% Contribution 1 - 100 words
\rev{\textbf{Design and implementation of a high-volume job power profiling and clustering pipeline for large scale HPC systems:}
We present the design and implementation of a job power profiling, indexing, clustering, and serving system that can handle high-volume telemetry data from large scale HPC systems and output resulting data as they come in.  The design of this system has been driven focused to reduce the time it takes to make use of the power profiles after data ingest, and then store \& serve the data to a few different classes of use-cases grouped by 1) low-latency interactive access, 2) batch consumption for machine learning model training and prediction, and 3) real-time consumption as a stream.  Here, we identify the general building blocks to support such a requirement and present the details.}

% Contribution 2 - 100 words
\rev{\textbf{Early experiences and lessons learned on feature extraction and unsupervised learning on HPC job profile data:}
Beyond the system itself, we also present the implementation details of the feature extraction and clustering of timeseries-based power profiles which are engineered to satisfy downstream applications and provide early experiences and lessons learned while embracing algorithms and techniques advanced from the data science community.  In particular, we identify and report the challenges we have found while employing “clustering”, a form of unsupervised learning, and ensuring the outcome is valid.}

% Contribution 3 - 100 words
\rev{\textbf{Early analysis on what we have found by grouping HPC jobs based on their features:}
Finally, we present an early analysis of what our clustering pipeline has found from the data we have used which was from the entire year of 2021, and demonstrate the correctness, usefulness, and areas of improvement helping ourselves establish a firm foundation for long-term operations and maintenance of the system.}


==> txt/backup/03_01_0_design_overview.tex <==
\section{Design and Implementation}
\label{sec:design}

\subsection{Design Goals}

\rev{
In this Section, we focus on three primary design goals for the job power profiling system: profiling based on high-resolution time series power measurement streams, ensuring low ingest-time-to-available delay and low latency access of profile data, and providing feature-driven labels for easy navigation. We elaborate on each of these design goals in the following sections, detailing our approach and techniques employed to achieve them.
}

\rev{
\subsubsection*{\textbf{Profiling based on high-resolution time series power measurement telemetry streams:}}
Our first design goal aims to provide contextualized job-level and component-level time series data from all jobs running on the HPC system. The objective is to capture the shape of the power profile, fluctuations, and swings from the job-level power consumption timeline.  To achieve this, we leverage a high-resolution out-of-band per-component and per-node power measurement from each node from the compute cluster~\cite{shin2021revealing, Thaler:2020, openbmc_event}.  To handle the high volume of such time series data and preserve the profiling output, we design our system to efficiently process, manage and store this information, enabling comprehensive analysis of power consumption patterns.
}

\rev{
\subsubsection*{\textbf{Low ingest-time-to-available delay and low latency access of historical profile data:}}
Recognizing that we are dealing with a data stream in motion rather than a static dataset, our second design goal aims to make downstream power profile data artifacts available as soon as possible after data ingestion. Also, we strive to make the data accessible within a reasonable interactive latency (i.e., under 3 seconds) when on-line historical profiling results are queried from applications.  To achieve this, we place a strong emphasis on data pre-processing to generate the profiling data artifacts.
}

\rev{
\subsubsection*{\textbf{Provide feature-driven labels for easy navigation:}}
Our third design goal focuses on providing better navigation into the data by grouping jobs based on the shape of their power consumption. We employ machine learning methods to offer enhanced navigation beyond the existing labels  of each job (i.e., user ids, project or account names, number of nodes and etc). By utilizing techniques that can extract features from the dynamics of the time series data, we can leverage these features to group jobs and index them based on their similarity. This approach enables users to easily navigate and explore the data, ultimately facilitating more effective analysis and decision-making.
}

%% - Data precreation
%% - Treat historical data & stream altogether
%% - Targeted feature extraction & data driven job classification (clustering)
%%   - Labels are not enough (projects, users & etc)

\subsection{End-to-end Pipeline}
\label{subsec:end-to-end}

\rev{
To achieve our objectives, we have implemented an end-to-end data pipeline on top of a system dedicated to data analytics applications, as illustrated in Figure~\ref{figs:arch}. Given the high volume of telemetry data streaming from our large-scale HPC systems, we utilize dedicated deployments of big data building blocks supported by an object store, providing the necessary compute power, memory, and storage. This pipeline targets and fully embraces the concept of streaming data as an ever-appending table, from its genesis to the end of its lifetime. Also, we pay special attention to ensuring flexibility in mutating and processing both new and historical data upon any policy change. To accommodate multiple downstream use-cases, this pipeline is designed to produce power profile data artifacts as a common resource across various applications. Keeping these goals and considerations in mind, we showcase the end-to-end pipeline of our work in Figure~\ref{figs:end-to-end}.
}

\rev{
\subsubsection*{\textbf{Data ingest:}}
Our system relies on a separate data engineering and data distribution system that is responsible for collecting telemetry data from heterogeneous sources into a single location and then distributing to downstream users as mentioned in Section~\ref{subsec:oda_arch}.  Among many telemetry data stream “topics”, our job power profiling mainly focuses on two data sources: 1) the job allocation data which comprises job allocation events \& node-level state change and 2) out-of-band high-resolution per-node, per-component (i.e., CPUs, GPUs) telemetry stream from the entire HPC cluster as seen in Figure~\ref{figs:end-to-end}-a).
}

\rev{
\subsubsection*{\textbf{Data processing:}}
Following data ingestion, the data undergoes extensive processing to suit downstream needs (Figure~\ref{figs:end-to-end}-b)). We focus on contextualizing power measurement data into a job allocation context by merging two data streams based on their timestamps and hostnames. This process includes data aggregation for timestamp alignment and pre-computation of variances and quantiles across various dimensions such as time, space, and allocated nodes. Pre-computations are performed at both job and component levels.  Due to the high-volume nature of the raw data ingest, we employ a dedicated data analytics cluster based on Apache Spark~\cite{spark} and leverage its structured streaming API~\cite{spark-structured-streaming} as a unified way of implementing data processing code for both new data in the streaming context (Figure~\ref{figs:end-to-end}-b) upper) and historical data (Figure~\ref{figs:end-to-end}-b) bottom) with a single copy of code.
}

\rev{
\subsubsection*{\textbf{Power profile database for serving:}}
Following the data processing step, the extensively refined data is ingested and served from a dedicated time series database (Apache Druid), which is specifically tuned for interactive querying and consumption (Figure~\ref{figs:end-to-end}-c)). This database primarily supports interactive web applications or dashboards with reasonable latency (i.e., under 3 seconds). Thanks to the pre-processing steps that utilize substantial memory and compute resources to reduce and summarize the data stream, the need for heavyweight queries that require reading and processing hundreds of thousands of rows in the synchronous path for interactive queries is eliminated. As new data is accumulated by the stream indexer, historical data can be reprocessed and ingested through a batch interface to update existing data in response to policy changes or data processing modifications in an idempotent manner.
}

\rev{
\subsubsection*{\textbf{Machine learning}}
The machine learning pipeline (Figure~\ref{figs:end-to-end}-d)) implements an automatic feature-based labeler. After processing 186 features from job-level timelines provided by previous stages, it utilizes an unsupervised learning-based clustering algorithm to classify HPC jobs by the similarity of total power consumption observed at the job level (i.e., only nodes allocated for that specific job during a certain duration). To reduce the time taken to produce such labels, we opted to train and deploy job classification predictors instead of directly using clustering algorithms. As outlined in Section~\ref{subsec:challenges}, clustering algorithms require reiteration of data from the beginning to produce output, which is unsuitable for a streaming context. Once trained, we capitalize on the relatively low computational cost of the model to "infer" labels based on what the model has learned from historical data. This model-based prediction of job labels is performed in either a streaming context for new data or a batch context for historical data, which is either published in the message bus for real time consumption or ingested into the time series database just like other components of the job power profile database.  Details of this stage are explained in Section~\ref{sec:implementation}.
}

\rev{
\subsubsection*{\textbf{Usage from applications and downstream}}
Once the two stages that involves data processing and machine learning (Figure~\ref{figs:end-to-end}-b) and d)) produce the outputs, the data is served towards downstream applications (Figure~\ref{figs:end-to-end}-e)) mainly in two ways based on application needs\footnote{Both methods provide near real time availability of most recent data, but would be provide different interface semantics or policies (i.e., data retention time) based on how it is deployed.}: one via the message bus for real-time consumption and another via the time series database (Figure~\ref{figs:end-to-end}-c) and d)\footnote{Same time series database instance}) for interactive consumption.
In general, a selected set of output data in the message bus would be redirected back to the center-wide data distribution system for a wider audience.  Also, the selected set would be served via wrapper REST APIs that proxies the native SQL interface of the time series database would make the data available for applications such as web-based user interfaces.
We aim to report results of downstream applications in our future works.
}


==> txt/backup/03_01_1_design_system_architecture.tex <==


\subsection{System Architecture}
\label{subsec:deployment}

%% Deployment
\input{figs/deployment}

Figure~\ref{figs:deployment-and-ops} illustrates the supporting system architecture for the end-to-end pipeline described in Section~\ref{subsec:end-to-end}. The pipeline is sustained by various data analytics and machine learning building blocks that offer the necessary storage and persistence, data forwarding, data processing compute power, experiment tracking, and workflow orchestration. These building blocks are deployed on a Kubernetes~\cite{kubernetes} cluster maintained by the user facility to support multiple internal applications.

\subsubsection*{\textbf{Data analytics cluster:}}
In response to the high volume generated by large-scale HPC clusters, we employ a dedicated Apache Spark-based data analytics cluster~\cite{spark}. This cluster leverages Spark's parallelization and handling capabilities for in-motion data streams and historical data.

\subsubsection*{\textbf{Persistence:}}
For data persistence, our system utilizes a dedicated S3 interface-based object store, MinIO~\cite{minio}, which serves as the primary backend-tier for persistence and capacity. The data pipelines running on the data analytics cluster rely on this persistence to manage data for offline batch processing workloads and historical data in its raw archived form, predominantly using Parquet~\cite{parquet} file formats for space and I/O efficiency required for historical data processing. Additionally, the time series database and machine learning model tracking service depend on this persistence as a backend to supply the necessary storage and maintenance of data and model artifacts from the pipeline.

\subsubsection*{\textbf{Workflow tracking, orchestration:}}
To manage the complexity of implementing multi-stage data processing tasks or intricate machine learning pipelines, we employ Apache Airflow~\cite{airflow} as our orchestration engine. Furthermore, for complex machine learning model training and maintenance workflows, we utilize MLFlow~\cite{mlflow}, a machine learning experiment and artifact tracking service that aids in managing workflow execution results and machine learning models.

\subsubsection*{\textbf{Machine learning models:}}
After training, machine learning models (e.g job classification predictors) are deployed into the model registry to be distributed to downstream batch job classification workflows or deployed via the inference server (RedisAI~\cite{redisai}) in a streaming context, generating new data. Once registered, the models are consumed by both batch and streaming contexts.


==> txt/backup/03_02_design_processing.tex <==
\section{Implementation Details}
\label{sec:implementation}

\subsection{Data Processing}
\label{subsec:data_process}

%% TODO: How we create the job profile database

\input{tables/data_spec}

Table~\ref{tab:data_spec} and Table~\ref{tab:der_data_spec} specify the inputs and outputs of the entire data processing pipeline described when it is in a historically archived compressed form (i.e., parquet files) in the backend filesystem for long-term offline processing, analysis, and development purposes.  With high-resolution data, the original input footprint is large, but through the processing done, the output turns out to be a modest size of approximately 2.0 TB for a year's worth of data.

There are largely four data sets as an outcome.  The first is the component level features which is the output of the first stage of the data processing (Table~\ref{tab:der_data_spec}-a)).  This stage turns high-resolution per-component data streams into a 10-second interval aggregation along with the time axis to cope with per-node timestamp errors. The second is the temporal component level data (Table~\ref{tab:der_data_spec}-b)) which partitions the timeseries into 10 equal bins irrespective of their lengths. We then aggregate the values for different
power and temperature components over each bin. Using the binning technique, we preserve the coarse-grained temporal context of timeseries. Third is the job level swing features (Table~\ref{tab:der_data_spec}-c)) which is 10 second timeseries in which we have calculated swing values upto 4 lags, i.e., we subtract the value at time $t$ by values at $t+1$, $t+2$, $t+3$ and $t+4$. This helps capture the swings in a timeseries over a larger window. Fourth is the job level swing range count (Table~\ref{tab:der_data_spec}-d)) which is job level highly aggregated data where we capture the top 5 swings in a positive and negative direction during the jobs complete runtime.
As these datasets are processed through the data pipeline, the resulting datasets are ingested into the time series database for downstream consumption.
%\ahmad{There are largely four data sets as an outcome.  The first is the component level features which is the output of the first stage of the data processing (Table~\ref{tab:der_data_spec}-a)).  This stage turns high-resolution per-component data streams into a 10-second interval aggregation along with the time axis to cope with per-node timestamp errors. The second is the temporal component level data (Table~\ref{tab:der_data_spec}-b)) which … TBD. Third is the job level swing features (Table~\ref{tab:der_data_spec}-c)) which is … TBD. Fourth is the job level swing range count (Table~\ref{tab:der_data_spec}-d)) which is … TBD.
As these datasets are processed through the data pipeline, the resulting datasets are ingested into the time series database for downstream consumption.

==> txt/backup/03_03_design_feature.tex <==
\subsection{Feature Extraction}
\label{subsec:features}

%%% TODO: supplementary illustration to explain what kinds of features we're talking about
%\input{figs/features}

%% TODO Data specification
%\input{tables/features_spec}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{plots/jobs_ts.pdf}
  \caption{Timeseries of typical HPC workloads. The plots help visualize that the features calculated in Table \ref{tab:data_feature_spec} can distinguish between different power profiles. Shades in each subplot correspond to 4 bins of timeseries. The labels assigned to these timeseries are shown below their x-axes.} 
  %\Description{Description of the image}
  \label{figs:sample-ts}
\end{figure}

%% Describe the process of ...
%% - feature extraction
%% - 

%\ahmad{\loremipsum{\textbf{150-words}- discuss what features are considered and how}} 

Feature extraction is a method by which relevant characteristics of data (power profiles) are calculated so that the data points with similar attributes reflect similar values for computed features. 
As earlier mentioned in section \ref{subsec:challenges-character}, power profile timeseries having varying lengths are characteristic of jobs that depend on the time length for which the HPC jobs ran. Varying timeseries are not ideally suited for ML algorithms as ML methods usually require all data points to have equal dimensions/lengths. Thus, feature extraction has added advantage, particularly in timeseries analysis and clustering, that length of extracted features vector will be the same for all power profiles and independent of the duration of the HPC jobs. 
From the HPC power facility's perspective, the two essential characteristics with the highest potential to adversely affect are the frequency of power swings and the range of magnitude of those swings. We focus on these two properties of power profiles for feature extraction. We also preserve the notion of temporal relevance when extracting the features by dividing the timeseries into four bins of equal time length. 

%\ahmad{\loremipsum{\textbf{150-words - how the features are extracted, examples} }}
As mentioned in the previous sub-section, two crucial characteristics of power timeseries are the frequency of swings and the magnitude of the range of swings. Part of the features we extracted was computed using the tsfresh package [cite?], and part was calculated using custom built-methods. We partitioned the timeseries of each workload into four bins as shown by four regions in each subplot of Figure \ref{figs:sample-ts}. The partitioning of timeseries into four bins allows us to maintain the temporal characteristics of power consumption signals. The binning of timeseries enables us to calculate the features for each bin in addition to aggregate values over the complete timeseries. Table \ref{tab:data_feature_spec} shows the summary of features that were extracted. We will describe a few features for brevity, and other features follow similar patterns. Feature \texttt{$[\text{*}]$\_mean\_input\_power} refers to the mean input power of four bins and is represented as \texttt{$\text{1}$\_mean\_input\_power}, \texttt{$\text{2}$\_mean\_input\_power}, \texttt{$\text{3}$\_mean\_input\_power}, and 
\texttt{$\text{4}$\_mean\_input\_power}. 
Similarly, feature \texttt{$[\text{*}]$\_sfq[p/n]\_$[\text{*}]$\_$[\text{*}]$} refers to rising and falling swings of all four bins and of magnitudes in the range of \texttt{50W-100W}, \texttt{100-200W}, \texttt{300-400W}, \texttt{400-500W}, \texttt{500-700W}, \texttt{700-1000W}, \texttt{1000-1500W}, \texttt{1500-2000W}, \texttt{2000-}\texttt{3000W}. 
Three of the sample features are: 1) \texttt{$\text{1}$\_sfqp\_$\text{50}$\_$100$} is a feature for bin one that counts rising swings in the range of \texttt{50W} to \texttt{100W}, 2) \texttt{$\text{1}$\_sfqn\_$\text{50}$\_$100$} is also a feature for bin one but counts falling swings in the range of \texttt{50W} to \texttt{100W} , and  3) \texttt{$\text{4}$\_sfqp\_$\text{1500}$\_$2000$} is a feature for bin four that counts rising swings in the range of \texttt{1500W} to \texttt{2000W}. \texttt{length} feature is calculated to normalize other features by dividing them by the length of the timeseries. It is because features having swing counts will have a larger value for longer timeseries, and a similar power profile will have a smaller swing count if the timeseries are shorter.. 
All of the features we calculated for profiling the power timeseries are either the magnitude of power values or swings in timeseries which helps us profile timeseries based on the most crucial features. 
\input{tables/features_list}

==> txt/backup/03_03a_gan.tex <==
\vspace{-2pt}
\subsection{Generative Adversarial Network (GAN)}
\label{subsec:gan}

%250 words
\input{figs/cluster_gan}
GANs have recently been deployed in various unsupervised learning and timeseries analysis projects~\cite{tadgan, clustergan, gan8594983}. GAN models provide a robust method to generate low-dimensional latent space $(\mathbb{R}_{z})$ representation of the high-dimensional $(\mathbb{R}_{x})$ real data and also captures the distribution of high-dimensional data. 
The GAN model we have used benefits from the techniques of modified GAN models because they have certain advantages over basic GAN model architecture~\cite{tadgan, clustergan, infogan, wasserstein}. 

The model in  Figure~\ref{figs:gan_arch}, in addition to Generator and Critique ($\texttt{C}_{a}$), also has Encoder and another Critique ($\texttt{C}_{b}$). The Generator maps the data from latent space$(\mathbb{R}_{z})$ to high-dimensional space($\mathbb{R}_{x}$) of real data. Critique ($\texttt{C}_{a}$), called discriminator in the basic GAN model, uses the Wasserstein method to calculate the loss in classifying real and generated data. Wasserstein loss helps the model overcome the mode collapse problem. Encoder encodes the data from the original space ($\mathbb{R}_{x}$) to the low dimensional latent space ($\mathbb{R}_{z}$). Critique ($\texttt{C}_{b}$) discriminates between random data and the encoded signal. It enables the Encoder to learn so as to generate the distribution of latent vectors, which recreate the real data with a distribution similar to the original distribution. The reconstruction-based method is useful in generating the dataset using a latent feature set. It also validates that the latent features of lower-dimensional data ($\mathbb{R}_{z}$) represent the information in higher-dimensional real data by showing that the distribution of the generated dataset is similar to the real data,
as shown in Figure~\ref{figs:gan_distribution}. 

The input to the GAN model, shown in Figure \ref{figs:gan_arch}, is the dataset (\texttt{X}) of extracted features vectors ($\mathbb{R}_x$) of size 186 and outputs latent vectors ($\mathbb{R}_z$) of size 20. The encoder model and the decoder model both have two linear layers and a batch normalization layer between the two linear layers. The input and output dimensions of the two encoder linear layers are 186x40 and 40x20 and the dimensions of the two decoder layers are 20x128, and 128x186. The activation function is \texttt{ReLU}. Critique's ($C_a$) three linear layers have input and output dimensions of 20x100, 100x10, and 10x1. Critique ($C_b$) has one linear layer  of input and output dimensions 20x1. 
\input{figs/distrbution_gan}

==> txt/backup/03_04_design_clustering.tex <==
\subsection{Job Clustering}
\label{subsec:clustering}

%% TODO: Supplementary figure or plot to  explain job clustering details

%% TODO TBD table for whatever use to describe details
%% of the clustering method and result
\input{tables/cluster_label_spec}
\input{tables/label_science_domain}

We perform a cross-sectional analysis of all the jobs running on the
leadership scale HPC system to get a holistic understanding of the power consumption behavior of HPC workloads. The objective is
to find the power patterns exhibited by various jobs running on the
HPC system, and also to predict patterns of the new jobs based on the learnings from already existing jobs' characteristics. In order to accomplish our objective, we first generated power consumption profiles for all HPC jobs using system-level power \& temperature data and application-level job scheduler logs, as described in Table~\ref{tab:data_spec} and Table~\ref{tab:der_data_spec}. We then use the clustering methods for pattern recognition and grouping of HPC workloads' based on their power consumption behavior. 

However, we need an annotated dataset to calculate the clustering accuracy. Some techniques, such as silhouette score~\cite{rousseeuw1987silhouettes} provide metrics for cluster performance without the labeled dataset. The method measures the association between cluster cohesion and cluster separation, and its value ranges from -1 to 1. However, the silhouette score provides relative values by which we can compare various clustering methods, but it does not provide absolute metrics like cluster coherency or accuracy. Therefore, an annotated dataset is critical for reliable analysis and ensuring metrics that can assess the quality of clusters in an absolute definition. 
To address the challenge of having annotated labels, we manually labeled around $846$ power timeseries of various patterns and assigned them to different classes. We, the researchers, did the annotation independently and then compared labels assigned to these timeseries. We kept the same label for the timeseries, where we assigned the same labels unanimously. For timeseries that were assigned conflicting labels, we labeled them based on the discussion.

We randomly selected and annotated $846$ timeseries of the HPC workload. The annotation or labeling of jobs was done at four levels. Sample timeseries with classification labels are shown in Figure~\ref{figs:sample-ts}. For example, Figure~\ref{figs:sample-ts}(a) has the label FF3-2, where FF3 corresponds to the profile pattern, and 2 corresponds to a magnitude of 2000 Watts. Every alphanumeric character corresponds to a level in the assigned classification label. In Figure~\ref{figs:sample-ts}(b), the class label is FP1-2, so at level L1, the annotation is F which is similar to the label of timeseries in Figure~\ref{figs:sample-ts}(a).  At level L2, in Figure~\ref{figs:sample-ts}(b) the annotation is FP, which differs from Figure~\ref{figs:sample-ts}(a). At level L3, the class label is FP1, and at level L4, the class label is FP1-2. The first three levels (L1, L2, L3) are based on the patterns, such as rising and falling swings and slopes. Labeling of level L4 is strictly based on the magnitude of the major region in the timeseries. L1 is the high-level or more coarse-grained level, and L2, L3 \& L4 are more fine-grained levels. The hierarchical classification of the dataset has several advantages. It enables us to visualize the classification of jobs at multiple resolutions. The L1 or high-level classifies the dataset into broader patterns and captures the most salient features exhibited by the HPC jobs. As we increase the classification level from L1 to L3, the basis of difference among the timeseries becomes more nuanced, capturing more subtle patterns in the timeseries. Finally, at level L4, if the two timeseries have a similar pattern but have different magnitudes, they are grouped into different classes depending on the magnitude. For the magnitude of timeseries, we have groups of 1, 2, 3, 4, 5, 6, and 7 for magnitudes of 2500W, 2000W, 1500W, 1200W, 1000W, 800W, and 600W respectively. For example, if we look at the plots in Figure~\ref{figs:sample-ts}, some plots are more similar compared to others. If we look closely, Figure~\ref{figs:sample-ts}(a) and Figure~\ref{figs:sample-ts}(b) have similar labels and belong to group F at L1, but at L4, their groups are FF3-2 and FP1-2, respectively. Similarly, Figure~\ref{figs:sample-ts}(c) and Figure~\ref{figs:sample-ts}(d) are similar at the L1 level as both belong to the J group, but as they are not exactly similar, Figure~\ref{figs:sample-ts}(c) at L4 is assigned JJ3-2 class Figure~\ref{figs:sample-ts}(d) is assigned JJ1-2 class. 

A summary of the class description of the four-level classification is given in Table~\ref{tab:describing_cluster_labels}. We also show the distribution of 846 samples across different groups at level L1 and the number of subgroups at L3 under each L1 group.
We also show the distribution of jobs from different science domains for level L1 in Table~\ref{tab:labeling_cluster_labels}. The distribution of jobs based on the science domain helps us understand at a high-level, the dominant power profiles exhibited by different areas.


% \cite{dimensionalityCurse1,dimensionalityCurse2}.

%\ahmad{\loremipsum{\textbf{150-words - TBD Paragraph 2} }}

%\ahmad{\loremipsum{\textbf{150-words - TBD Paragraph 3} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}


==> txt/backup/04_00_eval.tex <==
\section{Evaluation}
\label{sec:results}

%% TODO: Describe what we wanted to know from the design & implementation
In this section, we present the results obtained by applying the clustering method on the latent features of size 20. These features were generated using the GAN model applied to the 186 features listed inTable~\ref{tab:data_feature_spec}. We used the class homogeneity score to asses the performance of the clustering techniques. We also leveraged the k-means method for performing prediction tasks. 
%The significantly smaller dimension of the latent feature has a better performance and faster execution time. 
%\ahmad{\loremipsum{\textbf{100-words - Outline the settings \& evaluation} sit amet purus gravida quis blandit turpis cursus in hac habitasse platea dictumst quisque sagittis purus sit amet volutpat consequat mauris nunc congue nisi vitae suscipit tellus mauris a diam maecenas sed enim ut sem viverra aliquet eget sit amet tellus cras adipiscing enim eu turpis egestas pretium aenean pharetra magna ac placerat vestibulum lectus mauris ultrices eros in cursus turpis massa tincidunt dui ut ornare lectus sit amet est placerat in egestas erat imperdiet sed euismod nisi porta lorem mollis aliquam ut porttitor leo a diam sollicitudin tempor id eu nisl nunc mi ipsum faucibus vitae aliquet nec ullamcorper}}








==> txt/backup/04_01_eval_job_profiledb.tex <==
% \subsection{Job Profile Database}
% \label{subsec:results:prediction}

% %% TODO: Performance of the job profile database from a systems perspective Woong
% %% * Evaluates ingest bandwidth, throughput and latency
% %% * Evaluates inference throughput and latency

% \input{plots/example.tex}

% \woong{\loremipsum{\textbf{150-words - Evaluation 1. TBD} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

% \input{plots/example.tex}

% \woong{\loremipsum{\textbf{150-words - Evaluation 2. TBD} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

==> txt/backup/04_02_eval_training.tex <==
\subsection{Job Cluster Quality}
\label{subsec:results:optimizer}
%% TODO: Training pipeline performance, accuracy, training time, latency & etc.
%% TODO: Also justify the methodologies we're using (i.e., comparison between this and that)

%\input{plots/example.tex}

\input{plots/gan_cluster}

%\ahmad{\loremipsum{\textbf{150-words - Evaluation 1.}}}
We have used two clustering methods, namely k-means clustering and DBSCAN methods, to analyze the job power profile timeseries~\cite{kmeansMethod, dbscanMethod}.

We present the results obtained from the k-means cluster analysis with a value of $\text{K=70}$. We choose this value because the total number of unique labels that we have at level L3 is 70, listed in Table~\ref{tab:data_feature_spec}. We did not choose the value of $K$ corresponding to the number of unique L4 level because the number of clusters goes over 100, and some of the classes will have a few sample data. In addition, the classification profiles are primarily dominated by their pattern, i.e., level L1, L2, and L3. 
The results in the graphs in Figure~\ref{plots:gan_tru} show some plots from clusters with high homogeneity scores. The classes of four clusters in Figure~\ref{plots:gan_tru} are NN2-3, JJ3-2, HH2-3, and FP1-2, which are briefly described at a high-level in~Table\ref{tab:describing_cluster_labels}. Similarly, the plots of timeseries in Figure~\ref{plots:gan_mix} are from clusters that have timeseries from multiple clusters and homogeneity scores lower than those in Figure~\ref{plots:gan_tru}. For instance, in Figure~\ref{plots:gan_mix}(a), the clustering model grouped profiles having FF1-3 and OO1-3 labels into the same cluster. Similarly, other subplots in Figure~\ref{plots:gan_mix} have timeseries with different labels at level L4. If we observe closely, each of the timeseries in the plot in Figure~\ref{plots:gan_mix}(d) have different labels at L4, which are FF1-4, FF1-3, OA1-2, and FF4-2. However, for level L2, the two labels are FF and OA. This shows that the homogeneity value is higher at L2 compared to L4. Here, it is to be noted that the length of the timeseries does not affect the labels, and it is evident from Figures such as Figure~\ref{plots:gan_mix}(b), where the red and blue timeseries have the same label but different length. 

Results from the DBSCAN clustering are mainly shown in Figure~\ref{plots:gan_tru_dbscan}, and~\ref{plots:gan_mix__dbscan}. The plots in Figure~\ref{plots:gan_tru_dbscan} shows some of the classes that have high homogeneity score. If we compare the plots in Figure~\ref{plots:gan_tru_dbscan} (c) and Figure~\ref{plots:gan_mix}(c), we see that DBSCAN was able to better classify the class with the label MM at level L2. Figure~\ref{plots:gan_mix__dbscan} has classes that have a significant number of power profiles from more than one class. However, if we again observe closely, we will observe that the L1 level has higher homogeneity/coherency than L3 and L4. Figure~\ref{plots:gan_mix__dbscan} (a),~\ref{plots:gan_mix__dbscan}(b), and~\ref{plots:gan_mix__dbscan}(d) all have timeseries that belong to one class at L1 but are in different sub-classes at L4.

A few classes also had poor homogeneity scores in both k-means and DBSCAN clustering methods. The plots in Figure~\ref{plots:gan_error}(b) shows a class having timeseries with many different labels. Similarly, in Figure~\ref{plots:gan_error}(a) we show a class with a low homogeneity score for the DBSCAN method. 

The overall homogeneity score of the clusters for all four levels of classification is shown in Table~\ref{tab:eval_cluster_homogenety}. As expected, level L1 has the highest homogeneity score of 90\% and 84\% as it is the most general or high-level classification. Levels L3 and L4 have the least value of the homogeneity score because they correspond to a fine-grained classification level.

%\input{plots/example.tex}

%\ahmad{\loremipsum{\textbf{150-words - Evaluation 2.} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

%\input{plots/example.tex}

%\ahmad{\loremipsum{\textbf{150-words - Evaluation 3.} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}


\input{plots/gan_cluster_dbscan}
\input{tables/evaluation}
\input{plots/gan_cluster_error}


==> txt/backup/04_03_eval_clustering.tex <==
\subsection{Job Prediction Performance}
\label{subsec:results:behavior-analysis}

%% This is the Inference evaluation - job classification in real life
%% TODO: Realtime inference evaluation - cluster quality, classification latency

%\input{plots/example.tex}

%One of the main motivations of this work is to improve the power profile awareness of the HPC jobs in the real working environment. Prediction of the jobs power behavior is an effort towards that.   
Prediction is usually associated with supervised machine learning methods. However, as we do not have a large number of the labeled dataset, we could not build a supervised model that can be trained for classification tasks. In this effort, we leverage the k-means clustering method for the prediction task. The idea is that we should be able to predict the class labels of any new job that runs on the HPC. Out of about 846 labeled dataset, we split it into 80\% and 20\% using stratified sampling, provided there are sufficient data for that class. We used 80\% of the data for building the k-means clustering model. After k-means clustering is done, we use the cluster center proximity measure to assign labels to 20\% of the data. 
We performed the k-means clustering for different values of K for all four levels, homogeneity scores of which are shown by the heatmap in Figure~\ref{plots:heatmap}.  
The y-axis of the heatmap corresponds to the classes or labels of timeseries patterns, and the x-axis corresponds to different values of K in the k-means cluster. We search over a wide range of K values as seen in the x-axis of the four subplots of four different levels, shown in Figure~\ref{plots:heatmap}. The values in the heatmaps range from a
low score of 0 (blue) to a high score of 1(red). We can observe that
some of the classes have a high homogeneity score for some of the labels for almost all values of K represented by red colors. Some other classes have a low score for nearly all values of K represented by blue color. There are some classes for which the homogeneity
score changes based on the K values, as seen by changing colors in
some rows from blue to red. 

The prediction accuracy of the scores depends on the complexity of the timeseries. Some of the HPC jobs exhibit simple profiles with no complex swings or slopes, whereas others have random complex swings. The overall homogeneity scores of all classes for four levels for different values of K are shown in Table~\ref{tab:pred_score}.
%\input{plots/example.tex}

%\ahmad{\loremipsum{\textbf{150-words - Clustering result eval 2.} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

\input{plots/heatmap.tex}

\input{tables/pred_score}

==> txt/backup/05_related.tex <==
\vspace{-2pt}
\section{Related Works}

\subsubsection*{\textbf{Application power and energy profiling \& analysis:}} 
%\naw{\loremipsum{\textbf{100-words - Realtime ingest \& processing} 13 lines
Power and energy profiling and analysis \cite{shoukourian2014monitoring,shin2021revealing,gholkar2018pshifter} are important areas of research in the field of HPC applications, considering the development of energy-efficient HPC systems, important for a sustainable future. The authors do an in-depth and systematic analysis of the power data of the pre-exascale HPC system and provide insights into the energy consumption of the HPC applications, and the overall energy efficiency of the system \cite{shin2021revealing}. Power and energy analysis provides the opportunity to closely analyze application characteristics \cite{patel2020does} based on power profile \cite{feng2005power} and can provide optimization strategies to follow for energy efficiency \cite{wilde20144}.  
%}}

\subsubsection*{\textbf{Data driven job classification:}}
%\ahmad{\loremipsum{\textbf{100-words - Realtime ingest \& processing}
In recent years, there has been an increasing focus on utilizing data-driven methods to classify jobs in HPC systems \cite{bang2020hpc,fan2021dras}, which rely on machine learning techniques to evaluate the characteristics of jobs and predict job behavior (i.e. job duration \cite{naghshnejad2018adaptive,galleguillos2018data,wyatt2018prionn,mckenna2016machine}, job resource usage \cite{bose2021hpcgcn,emeras2017evalix,sirbu2016power,matsunaga2010use}, job scheduling \cite{galleguillos2020accasim,klusavcek2020alea}). \cite{presser2022towards} presents the feasibility of real-time classification of HPC workloads, where the focus is given to the detection of malicious HPC workloads, but the work lacks in having the experimental dataset, as malicious workloads were missing to perform their classification evaluation. The authors address the job classification problem \cite{tsujita2021job} of predicting two classes the high-power-consuming jobs and low-power-consuming jobs by using correlation analysis of job activities in CPU, memory, file I/O and compute node layouts using supervised classification models. In contrast, we focus on clustering jobs based on the jobs' power consumption and learn about different patterns the jobs exhibit, which is useful to predict the power consumption pattern of the incoming jobs. This work will also assist the HPC power facility with improved power awareness of the workloads.
%}}

\subsubsection*{\textbf{Timeseries clustering methods:}}
%\naw{\loremipsum{\textbf{100-words - Realtime ingest \& processing} 
Variable length timeseries clustering is an active area of research, and several methods have been proposed in recent years, differing in their distance measures \cite{muller2007dynamic,gharghabi2018matrix}, clustering algorithms, and applications \cite{amaral2022summertime}. There are two categories for timeseries clustering algorithms \cite{aghabozorgi2015time,liao2005clustering,alqahtani2021deep,javed2020benchmark}: raw-data-based or shape-based \cite{begum2015accelerating,paparrizos2017fast,wang2019hierarchical}, and feature-based \cite{tiano2021featts,tavenard2020tslearn,fulcher2017feature}, and our work falls into the latter one. \cite{trosten2019recurrent} presents a joint clustering and feature learning framework based on deep learning, where a recurrent network is trained to embed, each time series in a vector space such that a divergence-based clustering loss function can discover the underlying cluster structure, but it cannot handle timeseries with longer lengths due to the computational complexity of training the deep neural network. Though some of the recent works \cite{madiraju2018deep, ma2019learning} claim addressing variable length timeseries data in the paper, while closely looking at their code-base, we find that the model design does not support variable length timeseries. However, none of these works have shown experimental analysis with HPC operational data.   
%}}

==> txt/backup/06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsubsection*{\textbf{Knowing what you are looking for:}} 
\woong{\loremipsum{\textbf{150-words} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

\subsubsection*{\textbf{Challenges \& Opportunities:}} 
\woong{\loremipsum{\textbf{150-words} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

==> txt/backup/07_conclusion.tex <==
\section{Conclusion}

In this work, we have outlined the design and implementation of a job power profiling system capable of managing substantial volumes of telemetry data from a (pre-)exascale large-scale HPC system. This system provides contextualized behavioral representations of power consumption through job-level timeseries. We introduced a set of features that are calculated from the timeseries signal and have proven to be significant in classifying HPC job power profiles.
%The four-layer hierarchical annotation of the dataset was crucial in grouping the timeseries under different groups or subgroups at levels L1,  L2, L3, and L4. 
The hierarchical grouping allowed the two very different timeseries to be in two separate groups at level L1; at the same time, two similar signals having minor differences can be grouped under one class label at L1 but can have different class labels in the subgroups. It helped to preserve the magnitude of similarity or dissimilarity between any two timeseries. Furthermore, we utilized an unsupervised learning-based clustering approach to group jobs based on their similarities, enhancing navigation and understanding of the power envelopes. We also leveraged the clustering method to use it as a prediction for an incoming job's timeseries. We recognize the importance of job-level power profiles for various use cases and have designed this system to serve as a foundation for additional applications and use cases.



==> txt/backup/08_future.tex <==
\section{Future work}

\subsubsection*{\textbf{TBD Future Work Item:}}
dictumst quisque sagittis purus sit amet volutpat consequat mauris nunc congue nisi vitae suscipit tellus mauris a diam maecenas sed enim ut sem viverra aliquet eget sit amet tellus cras adipiscing enim eu turpis egestas pretium aenean pharetra magna ac placerat vestibulum lectus mauris ultrices eros in cursus turpis massa tincidunt dui ut ornare lectus sit amet est placerat in egestas erat imperdiet sed euismod nisi porta lorem mollis aliquam ut porttitor leo a diam sollicitudin tempor id eu nisl nunc mi ipsum faucibus vitae aliquet nec ullamcorper sit amet risus nullam eget felis eget nunc lobortis mattis aliquam faucibus purus in massa tempor nec feugiat nisl pretium fusce id velit ut tortor pretium viverra suspendisse potenti nullam ac tortor vitae purus faucibus ornare suspendisse sed nisi lacus sed viverra tellus in hac habitasse platea dictumst vestibulum rhoncus est pellentesque elit ullamcorper dignissim cras tincidunt lobortis feugiat vivamus at augue eget arcu dictum varius duis at consectetur lorem donec massa sapien faucibus et molestie ac feugiat sed lectus vestibulum mattis ullamcorper velit sed ullamcorper morbi tincidunt ornare massa eget egestas purus viverra accumsan in nisl nisi scelerisque eu ultrices vitae auctor eu augue ut lectus arcu bibendum at varius vel

dictumst quisque sagittis purus sit amet volutpat consequat mauris nunc congue nisi vitae suscipit tellus mauris a diam maecenas sed enim ut sem viverra aliquet eget sit amet tellus cras adipiscing enim eu turpis egestas pretium aenean pharetra magna ac placerat vestibulum lectus mauris ultrices eros in cursus turpis massa tincidunt dui ut ornare lectus sit amet est placerat in egestas erat imperdiet sed euismod nisi porta lorem mollis aliquam ut porttitor leo a diam sollicitudin tempor id eu nisl nunc mi ipsum faucibus vitae aliquet nec ullamcorper sit amet risus nullam eget felis eget nunc lobortis mattis aliquam faucibus purus in massa tempor nec feugiat nisl pretium fusce id velit ut tortor pretium viverra suspendisse potenti nullam ac tortor vitae purus faucibus ornare suspendisse sed nisi lacus sed viverra tellus in hac habitasse platea dictumst vestibulum rhoncus est pellentesque elit ullamcorper dignissim cras tincidunt lobortis feugiat vivamus at augue eget arcu dictum varius duis at consectetur lorem donec massa sapien faucibus et molestie ac feugiat sed lectus vestibulum mattis ullamcorper velit sed ullamcorper morbi tincidunt ornare massa eget egestas purus viverra accumsan in nisl nisi scelerisque eu ultrices vitae auctor eu augue ut lectus arcu bibendum at varius vel

==> txt/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsubsection*{\textbf{Knowing what you are looking for:}} 
\woong{\loremipsum{\textbf{150-words} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

\subsubsection*{\textbf{Challenges \& Opportunities:}} 
\woong{\loremipsum{\textbf{150-words} est sit amet facilisis magna etiam tempor orci eu lobortis elementum nibh tellus molestie nunc non blandit massa enim nec dui nunc mattis enim ut tellus elementum sagittis vitae et leo duis ut diam quam nulla porttitor massa id neque aliquam vestibulum morbi blandit cursus risus at ultrices mi tempus imperdiet nulla malesuada pellentesque elit eget gravida cum sociis natoque penatibus et magnis dis parturient montes nascetur ridiculus mus mauris vitae ultricies leo integer malesuada nunc vel risus commodo viverra maecenas accumsan lacus vel facilisis volutpat est velit egestas dui id ornare arcu odio ut sem nulla pharetra diam sit amet nisl suscipit adipiscing bibendum est ultricies integer quis auctor elit sed vulputate mi sit amet mauris commodo quis imperdiet massa tincidunt nunc pulvinar sapien et ligula ullamcorper malesuada proin libero nunc consequat interdum varius sit amet mattis vulputate enim nulla aliquet porttitor lacus luctus accumsan tortor posuere ac ut}}

==> txt/future.tex <==
\section{Future work}

\subsubsection*{\textbf{TBD Future Work Item:}}
dictumst quisque sagittis purus sit amet volutpat consequat mauris nunc congue nisi vitae suscipit tellus mauris a diam maecenas sed enim ut sem viverra aliquet eget sit amet tellus cras adipiscing enim eu turpis egestas pretium aenean pharetra magna ac placerat vestibulum lectus mauris ultrices eros in cursus turpis massa tincidunt dui ut ornare lectus sit amet est placerat in egestas erat imperdiet sed euismod nisi porta lorem mollis aliquam ut porttitor leo a diam sollicitudin tempor id eu nisl nunc mi ipsum faucibus vitae aliquet nec ullamcorper sit amet risus nullam eget felis eget nunc lobortis mattis aliquam faucibus purus in massa tempor nec feugiat nisl pretium fusce id velit ut tortor pretium viverra suspendisse potenti nullam ac tortor vitae purus faucibus ornare suspendisse sed nisi lacus sed viverra tellus in hac habitasse platea dictumst vestibulum rhoncus est pellentesque elit ullamcorper dignissim cras tincidunt lobortis feugiat vivamus at augue eget arcu dictum varius duis at consectetur lorem donec massa sapien faucibus et molestie ac feugiat sed lectus vestibulum mattis ullamcorper velit sed ullamcorper morbi tincidunt ornare massa eget egestas purus viverra accumsan in nisl nisi scelerisque eu ultrices vitae auctor eu augue ut lectus arcu bibendum at varius vel

dictumst quisque sagittis purus sit amet volutpat consequat mauris nunc congue nisi vitae suscipit tellus mauris a diam maecenas sed enim ut sem viverra aliquet eget sit amet tellus cras adipiscing enim eu turpis egestas pretium aenean pharetra magna ac placerat vestibulum lectus mauris ultrices eros in cursus turpis massa tincidunt dui ut ornare lectus sit amet est placerat in egestas erat imperdiet sed euismod nisi porta lorem mollis aliquam ut porttitor leo a diam sollicitudin tempor id eu nisl nunc mi ipsum faucibus vitae aliquet nec ullamcorper sit amet risus nullam eget felis eget nunc lobortis mattis aliquam faucibus purus in massa tempor nec feugiat nisl pretium fusce id velit ut tortor pretium viverra suspendisse potenti nullam ac tortor vitae purus faucibus ornare suspendisse sed nisi lacus sed viverra tellus in hac habitasse platea dictumst vestibulum rhoncus est pellentesque elit ullamcorper dignissim cras tincidunt lobortis feugiat vivamus at augue eget arcu dictum varius duis at consectetur lorem donec massa sapien faucibus et molestie ac feugiat sed lectus vestibulum mattis ullamcorper velit sed ullamcorper morbi tincidunt ornare massa eget egestas purus viverra accumsan in nisl nisi scelerisque eu ultrices vitae auctor eu augue ut lectus arcu bibendum at varius vel
